SatCLIP: Global, General-Purpose Location Embeddings with Satellite Imagery

Geographic information is essential for modeling tasks in fields ranging from ecology to epidemiology. However, extracting relevant location characteristics for a given task can be challenging, often requiring expensive data fusion or distillation from massive global imagery datasets. To address this challenge, we introduce Satellite Contrastive Location-Image Pretraining (SatCLIP). This global, general-purpose geographic location encoder learns an implicit representation of locations by matching CNN and ViT inferred visual patterns of openly available satellite imagery with their geographic coordinates. The resulting SatCLIP location encoder efficiently summarizes the characteristics of any given location for convenient use in downstream tasks. In our experiments, we use SatCLIP embeddings to improve prediction performance on nine diverse location-dependent tasks including temperature prediction, animal recognition, and population density estimation. Across tasks, SatCLIP consistently outperforms alternative location encoders and improves geographic generalization by encoding visual similarities of spatially distant environments. These results demonstrate the potential of vision-location models to learn meaningful representations of our planet from the vast, varied, and largely untapped modalities of geospatial data.

==> related_work.tex <==
\subsection{Spatial Context from Satellite Imagery}

% Satellite imagery has proven to be a valuable source of input data for predictive models across a wide range of applications \citep{Rolf2021}, for example, interpolating missing air pollution data \citep{Chen2019}, crop yield forecasting \citep{Tseng2022,lobell2015scalable}, and agro-forestry carbon stock prediction \citep{Reiersen2022}. In development settings, satellite-based machine learning models have helped to support humanitarian aid efforts by identifying dwellings in deprived areas \citep{Tiede2021,Wurm2019,Klemmer2020a}, predicting poverty \citep{Jean2016}, and mapping rural populations \citep{Hu2019}. 

But using satellite images in predictive models can be challenging: They can be difficult and computationally expensive to obtain, store, and analyze, especially in resource-constrained settings or at a global scale. As such, providing accessible and informative lower-dimensional feature representations based on satellite images has been a long-standing research topic in the remote sensing literature \citep{Quackenbush2004}. Traditionally, geometric and object-based filtering techniques have been utilized for this task \citep{Loos2002,Zhan2007}. More recently, \citet{Rolf2021} propose using random convolutional features extracted from global-coverage satellite imagery as a conceptually simple but highly effective geographic feature extractor for inexpensive, general use in downstream prediction tasks.

These prior methods all require imagery at the location-of-interest to extract features from. In contrast, we aim to capture spatial context with models that directly take geographic coordinates as the input--no image required. We do so by pretraining the location encoders to distill spatial variation in satellite imagery through contrastive pretraining. Our models thus learns to associate a given location with specific image characteristics.

\subsection{Contrastive Pretraining with Geospatial Data}

Unsupervised and self-supervised learning have become recent focuses for geospatial ML, as large portions of geospatial data--especially remotely sensed data like satellite imagery--are unlabeled \citep{Wang2022a}. The spatiotemporal nature of geospatial data can be exploited to construct unsupervised learning objectives based on contrasting inputs from different locations or times. For example, \citet{Jean2019} propose a triplet loss leveraging differences in nearby and far distant satellite image tiles for representation learning. \Citet{Manas2021} exploit seasonal differences in satellite images for model pretraining and highlight performance improvements over traditional ImageNet pretraining. 
\citet{scheibenreif2022self} and \citet{Wang2022b} pre-train models specifically on multi-spectral satellite data. To facilitate further progress in this direction, recent studies have also focused on creating and curating harmonized, multi-modal geospatial datasets \citep{Wang2022b, Lacoste2023}. However, all the mentioned efforts focus exclusively on pretraining vision encoders.

Three studies have pretrained geographic location encoders that input geographic coordinates, and return learned contextual representations. \Citet{Yin2019} propose GPS2Vec, a set of UTM-zone specific location encoders using geotagged Flickr images (YFCC100M) \citep{Thomee2016} and their corresponding semantic tags for training. Geographic generalization was out of scope for this work as embeddings are only available for UTM-zones in which training data can be found.
\Citet{Mai2023} introduce Contrastive Spatial Pre-Training (CSP) on the iNaturalist 2018 (iNat) \citep{Horn2018} species imagery and the Functional Map of the World (FMoW) \citep{Christie2018} satellite image datasets. 
CSP is used for unsupervised pretraining and downstream prediction on the same datasets and was not conceptualized for broader, global generalization across different tasks. Just like for GPS2Vec, the pretraining datasets, iNaturalist and FMoW, are unevenly distributed over space, with high image densities in North America and Europe and few images outside of Western regions. \Citet{Cepeda2023} propose GeoCLIP, in which the authors pretrain image and location encoders using the MediaEval Placing Tasks 2016 (MP-16) dataset \citep{Larson2017}, also consisting of geo-tagged Flickr images. However, their work focuses on applications in geolocating images and explorations of the trained image encoder, while our objective is to train global, general-purpose location encoders. 

In summary, existing work leaves two important gaps: understanding how location encoders generalize across various downstream tasks and ensuring global coverage during training.


==> tables/datasets_table_old.tex <==
\begin{tabular}{@{}cccccccc@{}}
\toprule
\textbf{Name} & \textbf{$n$} & \textbf{Spatial coverage} & \textbf{Locations} & \textbf{Outcome variable} & \textbf{Inputs} & \textbf{Task} \\ \midrule
\begin{tabular}[c]{@{}c@{}}Air Temp.\\ \citep{Hooker2018}\end{tabular} & $3,076$ & Global & Weather stations & \begin{tabular}[c]{@{}c@{}}Annual mean\\ temperature\end{tabular} & lon, lat & Regression \\
\begin{tabular}[c]{@{}c@{}}Med. Income\\ \citep{Jia2020}\end{tabular} & $3,107$ & Continental, USA & \begin{tabular}[c]{@{}c@{}}Census tract\\ centroids\end{tabular} & \begin{tabular}[c]{@{}c@{}}Median household\\ income\end{tabular} & lon, lat & Regression \\
\begin{tabular}[c]{@{}c@{}}Cali. Housing\\ \citep{KelleyPace2003}\end{tabular} & $20,640$ & California, USA & House locations & House price & lon, lat & Regression \\
\begin{tabular}[c]{@{}c@{}}Elevation (sampled)\\ \citep{Rolf2021}\end{tabular} & $99,995$  & Global & \begin{tabular}[c]{@{}c@{}}Regular sampled\\ locations\end{tabular} & Elevation & lon, lat & Regression \\
\begin{tabular}[c]{@{}c@{}}Pop. Dens. (sampled)\\ \citep{Rolf2021}\end{tabular} & $74,512$  & Global & \begin{tabular}[c]{@{}c@{}}Regular sampled\\ locations\end{tabular} & \begin{tabular}[c]{@{}c@{}}Population density\\ (logged)\end{tabular} & lon, lat & Regression \\
\begin{tabular}[c]{@{}c@{}}Countries\\ (Ours)\end{tabular} & $100,000$ & Global & \begin{tabular}[c]{@{}c@{}}Regular sampled\\ locations\end{tabular} & Country code & lon, lat & Classification \\
\begin{tabular}[c]{@{}c@{}}Biome\\  (Ours)\end{tabular} & $100,000$ & Global & \begin{tabular}[c]{@{}c@{}}Regular sampled\\ locations\end{tabular} & Biome type & lon, lat & Classification \\
\begin{tabular}[c]{@{}c@{}}Ecoregions\\  (Ours)\end{tabular} & $100,000$ & Global & \begin{tabular}[c]{@{}c@{}}Regular sampled\\ locations\end{tabular} & Ecoregion & lon, lat & Classification \\
\begin{tabular}[c]{@{}c@{}}iNat 2018\\ \citep{Horn2018}\end{tabular} & $460,406$ & Global & Image locations & Species classes & \begin{tabular}[c]{@{}c@{}}lon, lat,\\ image\end{tabular} & Classification \\ \bottomrule
\end{tabular}%

==> tables/methods_table_big.tex <==
\begin{table*}[t]
\centering\small
\caption{\textbf{Key characteristics of SatCLIP vs.\ the GPS2Vec, CSP and GeoCLIP location encoders and the MOSAIKS feature extractor.}}
\label{tab:overview}
\resizebox{\textwidth}{!}{ 
\begin{tabular}{ccccc}
    \toprule
    & \textbf{Spatial coverage}     & \textbf{Contextual data}            & \textbf{Location encoder}       & \textbf{Training objective} \\
    \midrule
        \multirow{ 2}{*}{\textbf{SatCLIP} (ours)}         & \multirow{ 2}{*}{Global (continuous)}                             & \multirow{ 2}{*}{S2-100K}                        & \multirow{ 2}{*}{Spherical harmonics \& Siren}   & \multirow{ 2}{*}{Cosine similarity of embeddings (CLIP)}     \\ 
    &                             &                  &    &                                 \\
    \multirow{ 2}{*}{\textbf{GPS2Vec} \cite{Yin2019}} 
     &    
     UTM-zone specific                      & YFCC images                     & \multirow{ 2}{*}{Two-level soft encoding}         & \multirow{ 2}{*}{KL-divergence of embedding distributions}  \\
                                           & (mostly Europe and N. America)  & and semantic tags              &                                 &                  \\
    \multirow{ 2}{*}{\textbf{CSP} \cite{Mai2023}}     & \multirow{ 2}{*}{Global (continuous) }                              & \multirow{ 2}{*}{FMoW, iNaturalist}               & \multirow{ 2}{*}{Sinusoidal transform \& FcNet}          & Cosine similarity of embeddings (CLIP)    \\
                                    &                                     &                                 &                        &+ negative location sampling + SimCSE\\
     \multirow{ 2}{*}{\textbf{GeoCLIP} \cite{Cepeda2023}}& \multirow{ 2}{*}{Global (continuous) }                              & \multirow{ 2}{*}{MediaEval 2016}                 & \multirow{ 2}{*}{Random Fourier Features \& MLP}   & \multirow{ 2}{*}{Cosine similarity of embeddings (CLIP)}                                \\
    &                             &                  &    &                                 \\
    \multirow{ 2}{*}{\textbf{MOSAIKS} \cite{Rolf2021}}& \multirow{ 2}{*}{Global (0.01$^\circ$ grid)}                              & \multirow{ 2}{*}{Planet Basemaps}                 & \multirow{ 2}{*}{N/A (direct feature extractor)}   & \multirow{ 2}{*}{None}                                \\
    &                             &                  &    &                                 \\
    \bottomrule
\end{tabular}
}
\end{table*}

==> tables/vision_models.tex <==
\begin{table}[b]
\caption{Comparisons of different vision encoders in the in-domain classification tasks. 
The full tables \cref{tab:res,tab:res_adaptation} can be found in the \cref{appendix:full_res}.
%Within each smoothness level L=10 or L=40, SatCLIP embeddings with all vision models achieve very similar accuracies on downstream tasks within 1-$\sigma$. Hence, all vision models are able to extract location-specific patterns.
}

    \label{tab:modelcomparison}
    \centering
\footnotesize
\resizebox{\textwidth}{!}{
\begin{tabular}{lrrrrrr}
\toprule
                   & ViT16,L=10        & ResNet18,L=10      & ResNet50,L=10     & ViT16,L=40         & ResNet18,L=40      & ResNet50,L=40      \\
                    \cmidrule(lr){2-2}  \cmidrule(lr){3-3}  \cmidrule(lr){4-4}   \cmidrule(lr){5-5}   \cmidrule(lr){6-6}  \cmidrule(lr){7-7}    
%Countries          & $93.97 \pm 0.30$  & $93.92 \pm 0.30$   & $94.28 \pm 0.18$  & $ 95.77 \pm 0.14$  & $ 95.92 \pm 0.10$  & ${96.00 \pm 0.14}$ \\
iNaturalist        & $65.69 \pm 0.50$  & $65.56 \pm 0.29$   & $65.50 \pm 0.43$  & ${65.98 \pm 0.61}$ & ${66.40 \pm 0.49}$ & ${66.03 \pm 0.54}$ \\
%Biomes             & $92.07 \pm 0.22$  & $92.10 \pm 0.23$   & $92.23 \pm 0.26$  & ${94.27 \pm 0.15}$ & ${94.33 \pm 0.10}$ & ${94.41 \pm 0.14}$ \\
Ecoregions         & $89.53 \pm 0.28$  & $89.57 \pm 0.23$   & $89.32 \pm 0.31$  & ${91.61 \pm 0.22}$ & ${91.53 \pm 0.15}$ & ${91.67 \pm 0.15}$ \\
\bottomrule
\end{tabular}}

\end{table}
